Open-vocabulary Video Question Answering: A New Benchmark for Evaluating the Generalizability of Video Question Answering Models

Video Question Answering (VideoQA) is a challenging task that entails complex multi-modal reasoning. In contrast to multiple-choice VideoQA which aims to predict the answer given several options, the goal of open-ended VideoQA is to answer questions without restricting candidate answers. However, the majority of previous VideoQA models formulate open-ended VideoQA as a classification task to classify the video-question pairs into a fixed answer set, i.e., closed-vocabulary, which contains only frequent answers (e.g., top-1000 answers). This leads the model to be biased toward only frequent answers and fail to generalize on out-of-vocabulary answers. We hence propose a new benchmark, Open-vocabulary Video Question Answering (OVQA), to measure the generalizability of VideoQA models by considering rare and unseen answers. In addition, in order to improve the model's generalization power, we introduce a novel GNN-based soft verbalizer that enhances the prediction on rare and unseen answers by aggregating the information from their similar words. For evaluation, we introduce new baselines by modifying the existing (closed-vocabulary) open-ended VideoQA models and improve their performances by further taking into account rare and unseen answers. Our ablation studies and qualitative analyses demonstrate that our GNN-based soft verbalizer further improves the model performance, especially on rare and unseen answers. We hope that our benchmark OVQA can serve as a guide for evaluating the generalizability of VideoQA models and inspire future research. Code is available at https://github.com/mlvlab/OVQA.

==> Figures/smoothing.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=\linewidth]{Figures/smoothing.png}
    \caption{\textbf{Comparison of before/after applying GNN-based soft verbalizer.}
    We illustrate the process of predicting the unseen answer `stroller' from the output feature of [MASK] token, $\mathbf{m}$.
    \textbf{(a) Before smoothing:} without the information of similar words from verbalizer, it is hard to predict the unseen answer.
    \textbf{(b) After smoothing:} with GNN-based soft verbalizer, the model is more likely to predict the unseen answers with the information of its neighborhoods (e.g., `chair' and `baby').
    }
    \label{fig:smoothing}
\end{figure}

==> Sections/backup/1_Introduction.tex <==
\section{Introduction}
\input{Figures/msrvtt/msrvtt}
\hjk{
Video question answering (VideoQA) is a multi-modal understanding task that requires complex reasoning between two modalities to find the correct answer given a video-question pair.
There are usually two task types in VideoQA, multiple-choice and open-ended.
The multiple-choice VideoQA requires the model to select the correct answer among several options.
On the other hand, in open-ended VideoQA, the model needs to predict the answer without restricting candidate vocabulary.

However, most existing VideoQA models~\cite{lei2021less,wang2022all,li2020hero,fu2021violet,zellers2021merlot,le2020hierarchical,yang2022zero} formulate the open-ended VideoQA task as a classification problem with a fixed set of answer candidates which frequently appear in the training set, \textit{e.g.}, top-1000.
Therefore, the out-of-vocabulary answers, not used during training, are automatically regarded as incorrect without any thorough consideration during evaluation.
Fig.~\ref{fig:answers} highlights that the top-1000 answer categories cover about 17.8\% of the answer candidates while they possess about 90.2\% of the total samples overwhelming those of other answer categories in Fig.~\ref{fig:samples}.
This suggests that previous models may show seemingly good performance only with \textit{top-k} answer candidates, yet they, in fact, fail to generalize to rare and unseen answers by ignoring the underrepresented out-of-vocabulary answers.
Such problems have been overlooked since these models have been evaluated in terms of overall performance only.
In other words, the conventional benchmark of open-ended VideoQA does not measure the generalizability and thus leads the model to neglect the realistic setting of class imbalance and unseen answers.
Therefore, a comprehensive benchmark that handles long-tail distribution with unseen answers is necessary.

% Previous models ignore the underrepresented out-of-vocabulary answers, and fail to generalize to unseen answers in real-world settings.
% This long-tail distribution problem is largely unexplored in open-ended VideoQA, and a comprehensive benchmark that deals with both class imbalance and unseen answers is necessary. 
% Fig.~\ref{fig:bar} illustrates the number of answers and triplets for each answer category. 
% Although the previous models discard the out-of-vocabulary answers, they have shown plausible performance since the dataset is extremely long-tailed (see Sec.~\ref{subsec:categorization} for details).
%This demonstrates that the models simply memorize the head answers and fail to generalize on the tail or unseen answers.
%In other words, previous approaches totally ignore the realistic setting of class imbalance and the presence of unseen answers.
%Hence handling long tail distribution with unseen answers is largely unexplored in open-ended VideoQA.

% Note Fig.~\ref{fig:dataset} represents the distribution of MSRVTT dataset in terms of the number of answers and of triplets.
%Specifically, Fig.~\ref{fig:msvd} highlights that the number of triplets possessed by top-1000 answers overwhelms them of other answer categories. 
% Specifically, Fig.~\ref{fig:msvd} illustrates the number of answers and triplets for each answer category. 
% The top-1000 answer categories cover about 18\% of the answer candidates while it possesses about 90\% of the total triplets overwhelming those of other answer categories.
% Thus, previous models have shown plausible performance but indeed overlooked relatively infrequent or unseen answer candidates on account of such an extremely long-tailed distribution,
% Therefore, we address that a new benchmark for evaluating the generalization performance of the model in a realistic setting of class imbalance dataset is necessary.
%In other words, previous models have indeed shown plausible performance but they have overlooked relatively infrequent or unseen answer candidates. (...). On account of such an extremely long-tailed dataset (...) it is essential to provide a new benchmark for evaluating the generalization performance of the model that covers the realistic setting of class imbalance.


Recently, prompt-tuning~\cite{schick2021exploiting,liu2021gpt,gao2021making,cui2022prototypical,shin2020autoprompt,schick2020automatically,holtzman2021surface,hu2022knowledgeable} has drawn increasing attention \dhk{in natural language processing (NLP)} due to its significant performance gain on zero-shot and few-shot learning in a parameter-efficient manner.
To fill the gap between the objectives of pretraining and fine-tuning, in prompt-tuning, the input texts of downstream tasks are converted to a \textit{cloze} form, consistent with the masked language modeling (MLM) objective leveraged in the pretraining phase.
Through the \textit{cloze}-style downstream task, the model is asked to fill in [MASK].
In addition, the concept of \textit{verbalizer} was introduced by \cite{schick2021exploiting} to manually bridge between the original label and its corresponding words to be filled in [MASK], \textit{e.g.}, filling the word `great' in [MASK] to predict the label POSITIVE in sentiment classification.
To replace the considerable human labor of hand-designed verbalizers, search-based verbalizers~\cite{gao2021making,schick2020automatically,shin2020autoprompt} are also proposed by searching the words automatically from training data.
Current works~\cite{cui2022prototypical,hambardzumyan2021warp,zhang2021differentiable} adopt soft verbalizers which consist of learnable tokens to find optimal embeddings during training.
However, although there are several efforts to find the ideal verbalizer, searching it for unseen answers is less dealt with.}

To this end, we introduce a new benchmark of open-ended VideoQA, named Open-vocabulary Video Question Answering (OVQA), to perform the task under a more real-world setting of long tail distribution with unseen answers.
In contrast to the previous approach of open-ended VideoQA which focuses only on frequent answers, OVQA requires the model to predict rare and out-of-vocabulary answers in addition.
Under OVQA, to address the problem that the models are highly biased toward frequent answers, we also propose a novel graph neural network (GNN)-based soft verbalizer to smooth the original answer embeddings by aggregating the information of similar words from an external knowledge base.
Specifically, the GNN-based soft verbalizer learns how to smooth the original answers with their neighborhood words in the training phase and is adapted to the test phase based on the learned smoothing function during training to enhance the prediction for the unseen answers.

% To achieve this, we first categorize the answers into four groups (base, common, rare, and unseen) based on the frequencies of $\langle$\textit{video}, \textit{question}, \textit{answer}$\rangle$ triplets in the training set.
% Our preliminary experiment on MSVD dataset with one of the strong open-ended VideoQA baselines, FrozenBiLM~\cite{yang2022zero}, demonstrates that the model is highly biased to the frequent answers, which achieves 72.7\% on base and 18.9\% on rare.

In our experiments, we develop OVQA baseline models with an additional answer encoder and improve their performances by taking into account rare and unseen answers as well.
Also, our extensive qualitative analyses and ablation studies demonstrate that GNN-based soft verbalizer adequately learns to smooth the original answers and improves the model generalizability by predicting the unseen answers along with their neighborhood information.

\noindent To sum up, our \textbf{contributions} are as follows:
\begin{itemize}
    \item[\textbullet] We propose a new benchmark of open-ended VideoQA, OVQA, to provide an opportunity to evaluate the model performance and its generalizability under the long-tail distribution of open-ended VideoQA including unseen answers.
    \item[\textbullet] We also present a novel GNN-based soft verbalizer to smooth the answers so that the model can be generalized on rare and unseen answers as well with their augmented similar words by an external knowledge base.
    \item[\textbullet] Our experiments show that the performance of our developed baselines with an additional answer encoder improved by further considering out-of-vocabulary answers.
    \item[\textbullet] Extensive ablation studies and qualitative analyses demonstrate that GNN-based soft verbalizer is a generally applicable algorithm which alleviates the issue that the model is highly biased toward frequent answers.
\end{itemize}










% To achieve this, we additionally adopt a text encoder such as CLIP~\cite{radford2021learning} and DeBERTa~\cite{he2020deberta} to extract answer features and calculate similarities between answer features and video-question multi-modal feature.
